Tactile-Proprioceptive Sensor Fusion for Contact Wrench Estimation in Whole-Body Physical Human-Robot Interaction

Direct physical guidance is a natural means of teaching and interacting with robots, and robotic skins make a key contribution by enabling sensitive contact sensing and localization. This paper presents a tactile-proprioceptive sensor fusion framework for natural physical human-robot interaction. Tactile cues from pneumatic skin pads serve as contact indicators that bypass the ambiguity between frictional residues and applied external forces, enabling highly sensitive contact detection without explicit friction identification. We fuse these cues with motor-current-based proprioception to reconstruct multi-axis contact forces on the robot surface. To maintain accuracy during motion, we employ a temporal convolutional network (TCN) to mitigate friction hysteresis during stick-slip transitions, reducing uncertainty at contact onset and yielding smooth, responsive guidance. We validate the approach on a skin-integrated robot arm: (i) multi-axis forces are reconstructed in stationary contacts, and (ii) simultaneous force estimation and kinesthetic teaching are demonstrated. Results indicate improved sensitivity and responsiveness across diverse contact conditions compared with tactile-only and proprioceptive-only baselines, supporting tactile-proprioceptive fusion as a reliable pathway to safe, intuitive physical human-robot interaction.

==> Chapter/04_Sensor_fusion.tex <==
\section{SENSOR FUSION}
    In robotic systems, the measured torque $\tau_{measure}$ is typically decomposed into several components, as shown in Equation \eqref{eq:ext_force}. This measured toque is often estimated from the motor current $I$, and a torque constant $K_t$ via Equation \eqref{eq:torque_current}.  
    \begin{equation}
        \tau_{measure} = \tau_{ext} + \tau_{dyn} + \tau_{fric}
        \label{eq:ext_force}
    \end{equation}
    \begin{equation}
        \tau_{measure} = K_{t} I
        \label{eq:torque_current}
    \end{equation}

    %(명확히 해야할 것 - contact aware는 모델프리 방법으로 정지상태에서만 사용 가능하고 tcn은 data driven으로 정적, 동적 모두 사용 가능함)
    \ks{Here,} $\tau_{fric}$ exhibits hysteresis in static and quasi-static regimes, which complicates modeling and reduces the accuracy of external force $\tau_{ext}$ estimation. To address this issue, this paper proposes two methodologies. %Subsection A presents a contact-aware method that 
    First, we exploits tactile signals to achieve fast and accurate external force estimation under static conditions. Next, \ks{we introduces a learning-based method to address uncertainty during static-to-dynamic transitions, enabling more natural motion in pHRI application, such as kinesthetic teaching.} %Building on this principle, Subsection B introduces a learning-based TCN that enhances estimation accuracy during static-to-dynamic transitions, enabling more natural motion in pHRI application as kinesthetic teaching.



\subsection{Contact-aware Joint Torque Estimation}

    % 정적 상태($\dot{q}=\ddot{q}=0$))에서의 외부 토크 추정을 위해, 촉각 센서의 접촉 이벤트를 활용하는 알고리즘을 제안한다. 이 알고리즘의 동작 조건은 시스템을 세 가지 상태로 정의하는 유한 상태 기계(Finite State Machine, FSM)로 정형화할 수 있다(Fig3). 각 상태는 다음과 같이 정의된다: **Static-NoContact**는 관절이 정지해 있고 외부 상호작용이 없는 대기 상태이며, **Static-Contact**는 정지 상태에서 외부 접촉이 등록된, 본 추정기의 동작 상태이다. 마지막으로 **Dynamic**은 관절이 움직이는 모든 경우를 포함하며, 정적 추정의 전제 조건이 만족되지 않는 상태이다. Contact-aware 알고리즘은 Static-NoContact에서 Static-Contact 상태로 전환될 때, 접촉 순간의 측정 토크$\tau_{measure}(t_{contact})$를 $\tau_{baseline}$으로 설정한다. 이때 Static-Contact 상태에 있는 동안, 외부 토크는 식 (3)을 통해 연속적으로 추정된다.
    \ks{First, we propose an algorithm to estimate external torque in static condition ($\dot{q}=0$) by exploiting contact cues from robotic skins}. \ks{The proposed algorithm can be formalized as a finite-state machine (FSM), as shown in Fig. 3. Here, we consider three states:}
    \vspace{6pt}
    
    \noindent \ks{(i) Static (without contact)\\: the robot is stationary and no external contact is detected.}
    \vspace{6pt}

    \noindent \ks{(ii) Static (with contact)\\: a contact is detected while the system remains stationary.}
    \vspace{6pt}
    
    \noindent \ks{(iii) Dynamic\\: the robot is in motion (i.e., physical interaction).}
    \vspace{6pt}
    
    \ks{At the moment of contact, the state in transitioned from (i) to (ii), and our algorithm performs torque disambiguation based on tactile cues.}
    %The operational conditions of this algorithm can be formalized by a Finite State Machine (FSM) that defines the system in three states (Fig. 3). Each state is defined as follows: Static-NoContact is the quiescent state where the joint is stationary and no external interaction is detected; Static-Contact is the operational state of our estimator, where external contact is registered while the system remains static. Finally, Dynamic includes all cases where the joint is in motion, and the preconditions for static estimation are not met. The contact-aware algorithm sets the measured torque at the moment of contact, $\tau_{measure}(t_{contact})$, as the baseline $\tau_{baseline}$ when transitioning from the Static-NoContact to the Static-Contact state. 
    While in the state (i), the external torque is continuously estimated via Equation \eqref{eq:torque_residual}.
    \begin{equation}
        \hat{\tau}_{ext} = \tau_{measure}(t) - \tau_{baseline}
        \label{eq:torque_residual}
    \end{equation}
    % 이러한 접근법은 고기어비 시스템 관측기에 필요한 추정 deadband을 효과적으로 제거하여 responsiveness을 향상시키는 주된 이점을 가진다. 접촉 순간의 큰 정지 마찰을 베이스라인에 포함시켜 온라인으로 상쇄함으로써, 기존 방식에서는 무시되었을 미세한 접촉력에 대한 민감도를 확보할 수 있다.
    \ks{This approach improves responsiveness in high-gear-ratio systems, where friction introduces large uncertainty. By canceling static friction at contact onset, we can bypass the large dead-band, which is required by other methods that rely purely on motor current and a dynamics model}
    %This approach has the primary advantage of improving responsiveness by effectively eliminating the estimation dead-band often required in observers for high-gear-ratio systems. 
    %By incorporating the large static friction at the moment of contact into the baseline for online cancellation, sensitivity to subtle contact forces, which would be ignored in conventional methods, can be secured.
    % 그러나 이 방법의 유효성은 정적 상태에 한정되며, fig3 의 Static-Contact에서 Dynamic 상태로의 전환 과정에서 발생하는 불연속성 문제를 내포한다. 정적으로 확립된 $\tau_{baseline}$은 동적 상태로 연속적으로 이어지지 못하며, 이로 인해 정지 마찰 한계(breakaway friction)를 넘어서는 순간 과도기적인 추정 오차가 발생한다. 이는 $\tau_{baseline}$이 암묵적으로 포함한 실제 정지 마찰 상태가 복잡한 friction hysteresis로 인해 동적 모델로 원활하게 전환되지 못하는 물리적 현상에 기인한다.
    
    However, this method is valid only in the static states (i) and (ii). Once motion is initiated using the estimated external force, the estimate collapses because a large discontinuity arises as friction transitions from static to kinetic. Consequently, the baseline torque $\tau_{baseline}$ obtained in the static state does not apply in the dynamic state (iii). This mismatch produces a large error that makes unnatural motion.
    %However, the validity of this method is confined to static states, and it entails a discontinuity problem during the transition from the Static-Contact to the Dynamic state in Fig.3. The statically established $\tau_{baseline}$ cannot be continuously extended into the dynamic state, leading to a transient estimation error at the moment of exceeding the breakaway friction. This is attributable to the physical phenomenon where the actual static friction state, implicitly included in $\tau_{baseline}$, does not transition smoothly to the kinetic friction regime due to complex friction hysteresis.
    
    
    % In static regimes ($\dot{q}=\ddot{q}=0$), we propose a contact-aware algorithm that separates model residuals from external forces using tactile sensing of contact events. Specifically, when an external contact is detected at time $t_{contact}$, the measured torque at that instant is set as the baseline $\tau_{baseline}$ to the measured torque at that instant: $\tau_{baseline}$ = $\tau_{measure}(t_{contact})$. This baseline effectively captures all pre-existing internal factors, including gravity and the prevailing static friction state at the moment of contact. Consequently, as long as the system remains static post-contact, the subsequent change in torque can be attributed purely to the applied external force. 
    % \begin{equation}
    %     \hat{\tau}_{ext} = \tau_{measure}(t) - \tau_{baseline}
    %     \label{eq:torque_residual}
    % \end{equation}

    % This model-free approach, leveraging sensor fusion, consequently provides the significant advantage of isolating external force without requiring an explicit static friction model. However, the validity of this approach is contingent upon the system remaining static. When the joint begins to move and transitions into a dynamic state ($\dot{q}\neq0$), the friction characteristics abruptly shift from static friction to kinetic friction. At this point, the static baseline $\tau_{baseline}$ becomes invalid. A naive switch to a conventional model-based estimation method would cause a significant discontinuity in the estimated external force, resulting from the sharp drop from static breakaway friction to kinetic friction.
    

    \begin{figure}[t!]
        \centering
        \includegraphics[width=3.3in]{Figure/figure_one_col.png}
        \caption{Contact aware FSM}
        \label{FSM}
    \end{figure}
        
\subsection{TCN-Driven Seamless Transition Compensator} %TCN-based Force Estimation
    To resolve the estimation discontinuity during static-to-quasi-static transitions, we proposed a \ks{AI-based} approach \ks{to compensate the transition hysteresis, which are not captured by the friction model \eqref{eq:static_fric}}. This leads to the following \ks{expression} for the external torque $\tau_{ext}$:
    \begin{equation}
        \hat{\tau}_{ext} = \tau_{measure} - (\tau_{dyn} + \tau_{fric} + \tau_{TCN})
        \label{eq:tcn_estimation}
    \end{equation}
     \ks{This approach directly uses the torque residual as a network input, so it provides richer information for modeling friction than relying solely on the kinematic states $q$, $\dot{q}$, $\ddot{q}$ only}. \ks{The network was trained on data collected in the absence of external forces, since applying external forces and obtaining ground-truth labels is challenging}
     %Since collecting data that includes external forces with ground truth is fundamentally difficult (e.g., due to the requirement for torque or force sensors and the complex experimental setup), training is typically performed with force-free data. 
     A critical consequence of this training strategy is that the model inherently cannot distinguish external forces from modeling errors, leading to erroneous compensation during online inference.
    \begin{figure}[t!]
        \centering
        \includegraphics[width=3.3in]{Figure/fig3_draft.png}
        \caption{TCN diagram}
        \label{figure label 03}
    \end{figure}
    
    To resolve this ambiguity, we employ a contact-aware latching mechanism that extends the principle from Subsection A. This mechanism latches the network's input upon contact detection, thereby preserving an input profile consistent with force-free training data. This isolation of pre-motion external force prevents the TCN from misinterpreting it as a model error to be compensated, ensuring the input profile during online inference remains consistent with that of the force-free training data. The operationalization of this approach comprises a data processing strategy for training and a conditional latching logic for inference, which are detailed subsequently.
    
    
    The network input tensor $X \in \mathbb{R}^{C_{in} \times L_{in}}$ %
    is composed of $\tau_{dyn}$ as well as the $q, \dot{q}, \ddot{q}$. The kinematic states are incorporated because quasi-static friction behavior generally depends on them \cite{paper27_presliding}. Additionally, the tensor contains the processed residual torque variable $\tau_{hidden}$ is defined as:
    \begin{equation}
        \tau_{hidden}(t) =
            \begin{cases}
                \tau_{measure}(t) - (\tau_{dyn}(t) + \tau_{fric}(t))& \text{if } \left|\dot{q}\right| \le \omega_{\text{ th}} 
                \\0 & \text{otherwise}
            \end{cases}
        \label{eq:hidden_torque_revised}
    \end{equation}

    The structure of Equation \eqref{eq:hidden_torque_revised} focuses the network's learning objective on the static-to-quasi-static transition by setting the input to zero during fully dynamic phases. This prevents the TCN from attempting to compensate for general dynamic model errors and concentrates network resources on modeling the stationary
    and transition regimes based on preceding static state information. To further enhance learning fidelity, a frequency separation strategy from \cite{paper13_PINN} is applied during training. Static-to-quasi static transitions often produce high-frequency components in the residual. Separating these high-frequency components allows the network to focus learning specifically on friction characteristics associated with the transition.

    The latching mechanism activates upon contact detection at $t_{contact}$. This action ensures that external forces applied after contact do not alter the input channel by modifying the base input signal $\tau_{hidden}(t)$ to a latched counterpart $\tau^{*}_{hidden}(t)$. This modification preserves input consistency, aligning the resulting online input profile with the force-free training data distribution, where the input remains static before motion onset, is formulated as follows:
    \begin{equation}
        \tau^{*}_{hidden}(t) = (1-L(t)) \cdot \tau_{\text{hidden}}(t) + L(t) \cdot \tau^*_{\text{hidden}}(t^{-}_{\text{contact}})
    \end{equation}
    where L(t) is a binary latch state variable that transitions from 0 to 1 at $t_{contact}$, and $\tau^{*}_{hidden}(t^{-}_{\text{contact}})$ represents the input value immediately preceding contact. 
      
    % This architecture ensures that the method's behavior in the static state is functionally equivalent to the principle described in Subsection A. Once latched, the TCN output stabilizes, creating a fixed baseline as follow:
    % \begin{equation}
    %     \tau_{dyn} + \tau_{TCN} \approx \tau_{baseline}
    %     \label{eq:torque_tcn_definite}
    % \end{equation}

    We propose an architecture that latches the network's input based on tactile contact information. This method ensures the network's static-state behavior is equivalent to the contact-aware principle in Subsection A. Furthermore, it provides a data-driven solution to the discontinuity problem inherent in transitions where static external force estimation must extend into dynamic situations, a key requirement in applications like kinesthetic teaching.



    % State-adaptive External Torque Estimation
        % contact 상황을 고려하여 joint torque를 계산
        % 정지마찰에 의한 term을 효과적으로 무시할 수 있음 (완벽하지는 않음)
        % FSM 기반 접근법이라고 봐야할 듯?
    % Temporal Convolutional Network 기반 수직 힘 추정
        % 공압 패드 출력 -> 수직힘으로 바로 계산하기엔 오차가 크다 (?)
        % 공압 패드 출력 + 모터 전류 값을 활용하여 수직 힘을 추정
            % 그런데 ground truth 역할을 하는 수직 힘은 어떻게 구함? 로드셀?
            % joint torque만으로 구한 수직힘을 과연 믿을만 한지는 생각해봐야...

    % 마찰 같은 온갖 잡귀가 덕지덕지 달라붙은 motor 정보를 pad 정보보다 더 신뢰할 수 있을지 모르겠음
    % pad가 관측 불가능한 성분을 motor 정보로 보완하는게 이 연구의 목적이지, 정확도를 높이는건 잘 모르겠음


    % \subsection{Uncertainty-gated Blending}
    % \lipsum[36-42]        
    % % Fuzzy logic 처럼 하겠다는 뜻인 듯? (difuzzification)
    % % 불확실도는 어떤 방식으로 얻을 생각인지?
    % % 접근 방법 자체는 좋으나 볼륨이 너무 커짐... 저널로 가야함...


    % Pad의 장점 1
        % contact 지점 인식 -> 정지마찰 term 우회
        % 작성 방향: 정지마찰의 문제점 언급 및 해결 방안 제시

    % Pad의 장점 2
        % motor current 방식의 한계 -> dynamic 상황에서의 오차 증대
        % pad 정보로 일부 완화 가능
        % 그럼 애초에 pad 왜 안쓰냐? -> (contact 상황에 따라 캘리브레이션이 달라지더라)
        % 작성 방향: 왜 굳이 정확하지 않은 motor current 정보를 쓸 수 밖에 없었는지를 설명 -> interaction 관점에서, contact 상황에 따라 calibration이 달라지는 문제가 더 크게 다가오더라... 차라리 중간중간 오차?가 발생하는건 참을만 하던데... -> 그래서 pad 안쓰고 motor 를 쓰기로 한거임.
        %%%% pad 정보와 motor 정보를 상호 보완해서 사용하겠다는 뜻 %%%%
    
    % 자연스러운 교시를 구현하는 것이 목적임을 염두하고 작성
